Geometry-aware RL for Manipulation of Varying Shapes and Deformable Objects

Manipulating objects with varying geometries and deformable objects is a major challenge in robotics. Tasks such as insertion with different objects or cloth hanging require precise control and effective modelling of complex dynamics. In this work, we frame this problem through the lens of a heterogeneous graph that comprises smaller sub-graphs, such as actuators and objects, accompanied by different edge types describing their interactions. This graph representation serves as a unified structure for both rigid and deformable objects tasks, and can be extended further to tasks comprising multiple actuators. To evaluate this setup, we present a novel and challenging reinforcement learning benchmark, including rigid insertion of diverse objects, as well as rope and cloth manipulation with multiple end-effectors. These tasks present a large search space, as both the initial and target configurations are uniformly sampled in 3D space. To address this issue, we propose a novel graph-based policy model, dubbed Heterogeneous Equivariant Policy (HEPi), utilizing $SE(3)$ equivariant message passing networks as the main backbone to exploit the geometric symmetry. In addition, by modeling explicit heterogeneity, HEPi can outperform Transformer-based and non-heterogeneous equivariant policies in terms of average returns, sample efficiency, and generalization to unseen objects. Our project page is available at https://thobotics.github.io/hepi.

==> ICLR_2025/Figure_Wrappers/appx_eval_equi_slide.tex <==
\begin{figure*}[t]
    \makebox[\textwidth][c]{
    \input{ICLR_2025/Figure_Wrappers/Legend/equi_five_methods}
    }
    \centering
    % First row of figures
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_cloth_hanging_equi/eval_full_Isaac-Cloth-Hanging-Multi-v0_eval_all.pdf}
        \caption{Original 3D Space}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_cloth_hanging_equi/eval_half_yaw_Isaac-Cloth-Hanging-Multi-v0_eval_all.pdf}
        \caption{$\theta_{\text{yaw}} \in (-\pi/2, \pi/2)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_cloth_hanging_equi/eval_quater_yaw_Isaac-Cloth-Hanging-Multi-v0_eval_all.pdf}
        \caption{$\theta_{\text{yaw}} \in (-\pi/4, \pi/4)$}
    \end{subfigure}
    
    \medskip
    % Second row of figures - centered by wrapping in a minipage
    \begin{minipage}{0.65\textwidth}
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_cloth_hanging_equi/appx_eval_quater_half_yaw_Isaac-Cloth-Hanging-Multi-v0_eval_all.pdf}
        \caption{$\theta_{\text{yaw}}\in (-\pi/8, \pi/8)$}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_cloth_hanging_equi/appx_eval_one_yaw_Isaac-Cloth-Hanging-Multi-v0_eval_all.pdf}
        \caption{Fixed orientation}
    \end{subfigure}
    \end{minipage}
    \caption{Performance of different models on the \emph{Cloth-Hanging} task across various sample spaces. Assuming the global scene located at $r=[0,1,0]^T$, then from left to right, we generate sample by rotating $r$ by (a) $\theta_{\text{roll}} \in (-\pi/4, \pi/2)$, $\theta_{\text{yaw}} \in (-\pi, \pi)$, (b) $\theta_{\text{yaw}} \in (-\pi/2, \pi/2)$, and (c) $\theta_{\text{yaw}} \in (-\pi/4, \pi/4)$. Meanwhile, the bottom row shows results for (d) $\theta_{\text{yaw}}\in (-\pi/8, \pi/8)$, and (e) the fixed orientation at $\theta_{\text{roll}}=0, \theta_{\text{yaw}}=0$. As the sample space decreases, performance improves across all models, with HEPi consistently outperforming the baselines. The additional plot with fixed orientation on the bottom are averaged over 5 seeds while the others with 10 seeds.}
    \vspace{-0.2cm}
    \label{fig:appx_eval_equi}
\end{figure*}


==> ICLR_2025/Figure_Wrappers/appx_rigid_pushing/noise_and_high_res.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{ICLR_2025/Figure_Wrappers/appx_rigid_pushing/eval_noise_heatmap_Isaac-Rigid-Pushing-No-Contact-Multi-v0_eval_all.pdf}
    \caption{\rebuttal{Sensitivity of HEPi to noise and input resolution in the \emph{Rigid-Pushing} task. Heatmaps display returns (darker indicates lower returns) under varying levels of artificial Gaussian noise in position and velocity inputs for low-resolution (\(<30\) nodes, left) and high-resolution (\(>1000\) nodes, right) object meshes. HEPi demonstrates robust performance across resolutions, with mild degradation under increased noise, highlighting its adaptability to noisy real-world environments.}}
    \label{fig:eval_noise_heatmap}
\end{figure*}

==> ICLR_2025/Figure_Wrappers/appx_rigid_pushing/task_description.tex <==
\begin{figure*}[t]
    \begin{minipage}{0.8\textwidth}
        \centering
        \begin{subfigure}[b]{0.3\linewidth}
            \includegraphics[width=\textwidth]{ICLR_2025/Figures/appx_rigid_pushing/rigid-pushing-task.png}
        \end{subfigure}
        \hspace{0.2cm}
        \begin{subfigure}[b]{0.45\linewidth}
            \includegraphics[width=\textwidth]{ICLR_2025/Figures/appx_rigid_pushing/eval_30_Isaac-Rigid-Pushing-No-Contact-Multi-v0_eval_all.pdf}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.1\textwidth}
        \centering
        \hspace{-1.5cm}
        \makebox[\textwidth][c]{
        \input{ICLR_2025/Figure_Wrappers/Legend/appx_three_method_vertical}
        }
    \end{minipage}
    
    \caption{\rebuttal{\textbf{Left:} Rigid-Pushing task, where a rod is controlled in the $x$-$y$ plane to push an object to a desired target position and orientation. \textbf{Right:} Performance comparison between HEPi and baseline models over 10 seeds. HEPi outperforms both baselines by effectively exploiting task symmetries and modeling heterogeneity.}
    }
    \vspace{-0.2cm}
    \label{fig:rigid_pushing_task}
\end{figure*}


==> ICLR_2025/Figure_Wrappers/eval_generalization_rigid_2_tasks.tex <==
\begin{wrapfigure}[18]{r}{0.475\textwidth}
  \vspace{-0.3in}
   \begin{center}
    \makebox[0.5\textwidth][c]{
    \input{ICLR_2025/Figure_Wrappers/Legend/two_methods}
    }

    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_generalization_rigid/eval_line_Isaac-Rigid-Sliding-Multi-v0_eval_unseen_onl3_wTAE_norect.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \includegraphics[width=\textwidth]{ICLR_2025/Figures/eval_generalization_rigid/eval_line_Isaac-Rigid-Insertion-Multi-v0_eval_unseen_onl3_wT_norect.pdf}
    \end{subfigure}
  \end{center}
  \vspace{-0.15in}
    \caption{Generalization performance on rigid-sliding and rigid-insertion tasks over 10 seeds. Models are trained on one object (\textit{plus}), two objects (\textit{plus}, \textit{star}), three object (\textit{plus}, \textit{star}, \textit{pentagon}) and tested on the remaining unseen objects. Graph-based models show better generalization than the Transformer, likely due to their ability to exploit object topology.}
    \label{fig:eval_generalization}
\end{wrapfigure}


==> ICLR_2025/Figure_Wrappers/eval_knn_vn_main.tex <==
\begin{wrapfigure}[15]{r}{0.3\textwidth}
  \vspace{-0.325in}
   % \vspace{-0.1in}
  \begin{center}
    \makebox[0.3\textwidth][c]{    \input{ICLR_2025/Figure_Wrappers/Legend/knn_v_five_methods_rope}
    }
    % \includegraphics[width=\linewidth]{ICLR_2025/Figures/eval_knn_vn_m2_Isaac-Rigid-Insertion-Multi-v0_eval_all.pdf}
    \includegraphics[width=\linewidth]{ICLR_2025/Figures/appx_theory/eval_knn_vn_m2_Isaac-Rope-Shaping-v0_eval_all.pdf}
    % \includegraphics[width=\linewidth]{ICLR_2025/Figures/appx_theory/appx_eval_knn_vn_m2_Isaac-Rope-Shaping-v0_eval_all.pdf}
  \end{center}
  \vspace{-0.2in}
    % \caption{Ablation with different k-nearest neighbors for \textit{obj-to-act} edges. Results are averaged over 8 seeds.}
    \caption{Ablation on \textit{Rope-Shaping} task with different k-nearest neighbors for \textit{obj-to-act} edges. Results are averaged over 8 seeds.}
    \label{fig:eval_knn_vn}
\end{wrapfigure}


